Timed Epistemic Knowledge Bases for Social Networks (Extended Version)

We present an epistemic logic equipped with time-stamps in the atoms and epistemic operators, which allows to reason not only about information available to the different agents, but also about the moments at which events happens and new knowledge is acquired or deduced. Our logic includes both an epistemic operator and a belief operator, which allows to model the disclosure of information that may not be accurate. Our main motivation is to model rich privacy policies in online social networks. Online Social Networks (OSNs) are increasingly used for social interactions in the modern digital era, which bring new challenges and concerns in terms of privacy. Most social networks today offer very limited mechanisms to express the desires of users in terms of how information that affects their privacy is shared. In particular, most current privacy policy formalisms allow only static policies, which are not rich enough to express timed properties like "my location after work should not be disclosed to my boss". The logic we present in this paper enables to express rich properties and policies in terms of the knowledge available to the different users and the precise time of actions and deductions. Our framework can be instantiated for different OSNs, by specifying the effect of the actions in the evolution of the social network and in the knowledge disclosed to each agent. We present an algorithm for deducing knowledge, which can also be instantiated with different variants of how the epistemic information is preserved through time. Our algorithm allows to model not only social networks with eternal information but also networks with ephemeral disclosures. Policies are modelled as formulae in the logic, which are interpreted over timed traces representing the evolution of the social network.

==> instantiation-snapchat.tex <==
% !TEX root = ../main.tex
% !TEX macros = ../macros.tex
In order to mode the specificities of concrete social network systems we
introduce the notion of instantiation.

\begin{definition}
  A \rtfppf~instantiation for an SNS $\mathcal{S}$ is a tuple of the form:

  $\rtfppf^{\mathcal{S}} = $
  where $\sni{S}^{\mathcal{RT}} =
         \langle
            \agi{S}, \structi{S}, \kbii{S}, \poval_{\mathcal{S}}
         \rangle$
  and
  \begin{itemize}
    \item
  \end{itemize}
\end{definition}

